Memory Management in Resource-Bounded Agents

In artificial intelligence, multi agent systems constitute an interesting typology of society modeling, and have in this regard vast fields of application, which extend to the human sciences. Logic is often used to model such kind of systems as it is easier to verify the explainability and validation, so for this reason we have tried to manage agents' memory extending a previous work by inserting the concept of time.

==> eptcsdata.tex <==
\providecommand{\firstpage}{452}
\providecommand{\publicationstatus}{B. Bogaerts, E. Erdem, P. Fodor, A. Formisano,\\ 
G. Ianni, D. Inclezan, G. Vidal, A. Villanueva, \\
M. De Vos, F. Yang (Eds.): International \\
Conference on Logic Programming 2019 (ICLP'19).\\
EPTCS 306, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.306.61}{10.4204/EPTCS.306.61}}

